ChromoSkein: Untangling Three-Dimensional Chromatin Fiber With a Web-Based Visualization Framework

We present ChromoSkein, a web-based tool for visualizing three-dimensional chromatin models. The spatial organization of chromatin is essential to its function. Experimental methods, namely Hi-C, reveal the spatial conformation but output a 2D matrix representation. Biologists leverage simulation to bring this information back to 3D, assembling a 3D chromatin shape prediction using the 2D matrices as constraints. Our overview of existing chromatin visualization software shows that the available tools limit the utility of 3D through ineffective shading and a lack of advanced interactions. We designed ChromoSkein to encourage analytical work directly with the 3D representation. Our tool features a 3D view that supports understanding the shape of the highly tangled chromatin fiber and the spatial relationships of its parts. Users can explore and filter the 3D model using two interactions. First, they can manage occlusion both by toggling the visibility of semantic parts and by adding cutting planes. Second, they can segment the model through the creation of custom selections. To complement the 3D view, we link the spatial representation with non-spatial genomic data, such as 2D Hi-C maps and 1D genomic signals. We demonstrate the utility of ChromoSkein in two exemplary use cases that examine functional genomic loci in the spatial context of chromosomes and the whole genome.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/2d-vs-3d.tex <==
\tochangenote{might make sense to shorten and place elsewhere}
\dk{Before describing the design of our proposed tool, we discuss the value of linear (\ie, 1D or 2D) representation and its spatial (\ie, 3D) counterpart. We specifically compare 3D structures prediction with a heatmap representation coming from the Hi-C experiment.}










%% \annot{possible interactions}
%% \dk{Interactions in 1D and 2D based tools have become standardized, mainly also thanks to their similarities to everyday-use applications such as online maps. All 1D and 2D genomic tools for example feature zooming and panning interaction.}



==> sections/results-and-discussion.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/sketches/Paper.png}
    \caption{\mt{1. Support for overlaying multiple 3D data. Density shown here. These bins are made into a selection and added as a track next to distance. 2. Spherical selection encompassing structural change between A and B. Selection is added as a 1D track next to distance map. 3. Users can add custom 1D tracks, for example genes locations. All of these can be correlated together with selections to get insight into areas of interest.}}
    \label{fig:my_label}
\end{figure*}


